GANTEE: Generative Adversatial Network for Taxonomy Entering Evaluation

Taxonomy is formulated as directed acyclic concepts graphs or trees that support many downstream tasks. Many new coming concepts need to be added to an existing taxonomy. The traditional taxonomy expansion task aims only at finding the best position for new coming concepts in the existing taxonomy. However, they have two drawbacks when being applied to the real-scenarios. The previous methods suffer from low-efficiency since they waste much time when most of the new coming concepts are indeed noisy concepts. They also suffer from low-effectiveness since they collect training samples only from the existing taxonomy, which limits the ability of the model to mine more hypernym-hyponym relationships among real concepts. This paper proposes a pluggable framework called Generative Adversarial Network for Taxonomy Entering Evaluation (GANTEE) to alleviate these drawbacks. A generative adversarial network is designed in this framework by discriminative models to alleviate the first drawback and the generative model to alleviate the second drawback. Two discriminators are used in GANTEE to provide long-term and short-term rewards, respectively. Moreover, to further improve the efficiency, pre-trained language models are used to retrieve the representation of the concepts quickly. The experiments on three real-world large-scale datasets with two different languages show that GANTEE improves the performance of the existing taxonomy expansion methods in both effectiveness and efficiency.

==> 01_Introduction.0.tex <==
% Taxonomy is a particular type of hierarchical knowledge graph that portrays the hypernym-hyponym relations or ``is-A'' relations of various concepts and entities. 
% They have been adopted as the underlying infrastructure of a wide range of online services in various domains, such as product catalogs for e-commerce \cite{luo2020alicoco}, scientific indices like MeSH \cite{lipscomb2000MeSH}, lexical databases like WordNet \cite{miller1995wordnet}, product taxonomies built by Amazon \cite{dong2020autoknow} and universal concept databases Probase \cite{wu2012probase,chen2019cnprobase}. 
% A well-constructed taxonomy can assist various downstream tasks, including web content tagging \cite{liu2020giant,liu2019tencent_taxonomy,peng2019RCNN4taxonomy}, personalized recommendation \cite{karamanolakis2020txtract, huang2019taxonomy, zhang2014taxonomy}, query understanding  \cite{yang2020co, hua2016understand} and so on. 
Taxonomy is formulated as directed acyclic graphs or trees, which consist of \emph{hyponym-hypernym} relations between concepts.
One concept is a hypernym of another concept if the meaning of the former covers the latter\cite{sang2007extracting}.
% Many taxonomies are adopted as the underlying infrastructure of a wide range of online services, such as product catalogs for e-commerce \cite{luo2020alicoco}, scientific indices like MeSH \cite{lipscomb2000MeSH}, lexical databases like WordNet \cite{miller1995wordnet}, product taxonomies built by Amazon \cite{dong2020autoknow} and universal concept databases Probase \cite{wu2012probase,chen2019cnprobase}. 
A well-constructed taxonomy can assist various downstream tasks, including web content tagging \cite{liu2020giant,liu2019tencent_taxonomy,peng2019RCNN4taxonomy}, personalized recommendation \cite{karamanolakis2020txtract, huang2019taxonomy, zhang2014taxonomy}, query understanding  \cite{yang2020co, hua2016understand} and so on. 

% 1. A是啥，很重要。
% 2. expansion是维护A不断增长一种重要方式。
% 3. 然而，他们并没有考虑Taxonomy Entrance Evaluation，会所带来以下三点的后果：1）效果不好。2）开销大。
% 4. 在本文。我们提出一个即插即用的评估组件，off-the-shelf，放在expansion任务之前。输入A和taxonomy，我们首先判断A是否能挂在到taxonomy上，然后执行现有的expansion模型将其挂在到某一节点中。我们之所以引入这个组件的原因有以下2点：1）2）
% 5. To this end, 我们设计了。。。模型来实现这一组件。1）有监督，需要注意两个点：一是否是一个概念，二概念是否合适，这部分设计为。。分类方法。2）由于是有监督方法，需要负样本，伪标签，confuing，因此需要。。生成模型。3）为了将1）和2）joint，我们利用gan。。
% 6. 看实验效果：第一句。将组件加到10个方法中，实现了新sota。分别在数据集A，B提升了多少。并且在效率上加快了多少。并且在哪上线。。API。。

% 1. task新
% 2. 新方法
% 3. 效果好，效率快

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{introduction.png}
    \caption{An example of the new framework of taxonomy expansion task combined with the Taxonomy Entrance Evaluation task}
    \label{fig:introduction}
    \vspace{-5mm}
\end{figure}

Manually constructing and maintaining a taxonomy is labor-intensive, expensive, and time-consuming.
So the task of automated taxonomy expansion is hence proposed \cite{jurgens2016semeval},  which aims to automatically assign an existing concept (anchor concept) as a hypernym concept to the newly input concept (query concept).
The mainstream taxonomy expansion methods tend to use the self-supervised method to generate data from the existing taxonomy \cite{shen2020taxoexpan, yu2020steam, wang2021enquire, zhang2021taxonomy, mao2020octet, ma2021hyperexpan, wang2022qen}.
The accuracy of the automatic-annotated data is highly guaranteed, and the cost of both time and expense is much lower than previous methods.

\red{
However, these traditional taxonomy expansion methods only focus on calculate the similarity between each anchor concept to the query concept\cite{shen2020taxoexpan, yu2020steam, zhang2021taxonomy, wang2021enquire, wang2022qen}, and ignore the problem of whether the query concept should be added to the existing taxonomy at all.
These two tasks sound similar, but we consider they are different.
As we show in Figure \ref{fig:introduction}, when input ``The Eiffel Tower'' and ``Coconut Cake'' to the taxonomy of ``Computer Science'', previous methods will only calculate the similarity between the query concept to each of the anchor concept.
However, the similarity between anchor concept and unknown query concept are greatly determined by the initial representation of the query concept, and learning a good representation for all query concepts may be a huge expense since there are unlimited potential query concepts in real-scenrios.

without specific training, the similarity between unknown query concept and existing anchor concept are random, so even the input query concepts are noisy, the traditional taxonomy expansion model will probabily calculate a high similarity to it.
As in the real scenario, the query concepts are often noisy, as far as we know, none of the previous researches have studied such questions before, most of the researches just build self-supervised datasets which ignore it at all.
The consequence of ignoring such problem will cost another large labor-intensive expense to manually denoise the query concepts before the taxonomy expansion, since the taxonomy expansion model do not have the ability to distinguish the noisy. 
% The consequence of ignoring such problem is listed as follows:
% \begin{itemize}
%     \item The model does a poor job in distinguishing the noisy query concept from the clean query concept since it does train on such task at all.
%     \item When inputting large-scale noisy query concepts, it is still consuming much time to denoising such query concepts on manual work.
% \end{itemize}
}


% In this paper, we propose a new task called taxonomy enterance evaluation, which aims at evaluating whether a query concept should be added to the existing taxonomy or not.
% To solve this question, \red{negative data are needed.}
% The traditional taxonomy expansion method do not 

In this paper, we propose a new task, called taxonomy enterance evaluation, together with a corresponding method called Generative Adversarial Network for Taxonomy Enterance Evaluation (GANTEE).
Before the taxonomy expansion, we use GANTEE to evaluate whether a query concept should be added to the existing taxonomy.
And then the existing taxonomy evaluation methods are used to assign an anchor concept to the query concept.
The reasons why we introduce GANTEE are listed as follows:
\begin{itemize}
    \item GANTEE will make the model have a strong ability to distinguish the noisy query concepts.
    \item When the number of query concepts is large, the denoise method will best increase the efficiency of the whole process.
\end{itemize}

A pre-trained auto-regressive generative model is used in GANTEE to introduce the outside information to alleviate the above problems.
Beyond that, a pure auto-regressive is mainly used to generate sentence-level text, and the semantic of concept, which is word-level text, is hard to be captured.
So the extra supervised signal is needed to guarantee the generated text is a concept that has a hyponym relation to the given anchor query.

To this end, we use Generative Adversarial Network(GAN) \cite{goodfellow2014generative} to alleviate the above problem.
Specifically, in GAN a discriminative net $\mathcal{D}$ learns to tell the fake data apart from the real data, and the generative net $\mathcal{G}$ learns to confuse $\mathcal{D}$ by generating fake data which has similar distribution with the real data.
We take the generative model as a reinforcement learning agent; the state is the generated tokens combined with the prior information of anchor concepts, and the action is the next token to be generated.
The generated texts are expected to be a fake query concept which is a hyponym to the given anchor concept, but a question proposed by the previous research\cite{guo2018leakgan} that when the discriminator is too strict, the effective gradient won't be calculated, so we use a loose rollout discriminator and a strict hyper discriminator to provide supervised generative signal during the generating process.
Rollout process \cite{yu2017seqgan} is proposed to alleviate the problem of gradient passing back, which is used to guarantee that the generated text is a concept during the generating process.
A hyper discriminator is used to detect whether the generated query concept has a ``hyponym'' relation to the given anchor concept after the generating process.

In the experiments, we benchmark the taxonomy entrance evaluation task on three real-world taxonomies in two different languages, English and Chinese.
We make new State-Of-Art score in the experiments by improve the hit@1 from \red{xxx} to \red{xxx}, MR from \red{xxx} to \red{xxx} and MRR from \red{xxx} to \red{xxx}.
Then we test the efficiency of our method, and GANTEE still outperforms the baselines by a large margin on all three datasets.
Finally, extensive experiments have been conducted to study how the parameters affect the result of GANTEE, and provide an effective tuning scheme for the following researchers who will use our method in the future.

\subsubsection{Contribution.}
To summarize, our major contributions include: 
(1): a more realistic task called taxonomy entrance evaluation which judges whether a query concept should be added to an existing taxonomy or not;
(2): a novel, effective, and PnP method called GANTEE to generate graph-level negative samples which boosts the performance and the efficiency for both traditional taxonomy expansion tasks and taxonomy enterance evaluation tasks.
(3): extensive experiments that verify the effectiveness of GANTEE on three datasets in two languages, and an effective tuning method was proposed by the experiment.

% Manually constructing and maintaining a taxonomy is laborious, expensive, and time-consuming. 
% It is also highly inefficient and detrimental for downstream tasks if we construct a taxonomy from scratch \cite{gupta2017taxonomy, velardi2013ontolearn} as long as the taxonomy has new terms to be added. A more realistic strategy is to insert new terms (“query”) into an existing taxonomy, i.e., the seed taxonomy, as a child of an existing node in the taxonomy (“anchor”) without modifying its original structure to best preserve its design. 
% This problem is called taxonomy expansion \cite{jurgens2016semeval}.  


% Early taxonomy expansion approaches use supervised methods that annotate the terms which do not exist in the existing taxonomy to the position it should be added \cite{jurgens2015reserating}.
% Such approaches suffer from the insufficiency of training data and also a huge expanse of human effort.
% Recent studies concentrate on self-supervised method to generate data from the existing taxonomy automatically \cite{shen2020taxoexpan, yu2020steam, wang2021enquire, zhang2021taxonomy, mao2020octet, ma2021hyperexpan, wang2022qen}.
% The accuracy of the automatic-annotated data is highly guaranteed, and the cost of both time and expanse are much lower than previous methods, the most of all, they achieve great success in the experiments.
% Nowadays, such self-supervised methods have thus become the mainstream of the taxonomy expansion task.

% \red{
% However, the existing methods of taxonomy expansion task are mainly focus on how to give the best anchor concept to the query concept,  regardless of whether the query concept should be added into the existing taxonomy.
% In the real-scenario, the query concepts are often noisy, while the previous studies in industry application use rule-based methods to denoise the input data\cite{cheng2022learning}, most of the studies just build self-supervised datasets which ignore such question at all\cite{shen2020taxoexpan, yu2020steam, zhang2021taxonomy, wang2021enquire, wang2022qen}.
% The mainstream methods are lack of the ability to distinguish whether a query concept should be added into the taxonomy because they generate training data from the existing taxonomy only, the noisy data are not included during the training process.
% These sampled data are all node-level samples, which only used to denote whether two nodes have an ``isA'' relation or not.
% More graph-level negative data are needed to train a model which can tell whether a node should be added to the taxonomy or not.
% }

% Generatie Adversarial Network(GAN) \cite{goodfellow2014generative} is a promising framework for alleviating the above problem.
% Specifically, in GAN a discriminative net $\mathcal{D}$ learns to tell the fake data apart from the real data, and the generative net $\mathcal{G}$ learns to confuse $\mathcal{D}$ by generating fake data which has similar distribution with the real data.
% This approach was successful in computer vision tasks, then was transformed into natural language process and also achieved great success \cite{yu2017seqgan, guo2018long, wang2018sentigan, nie2018relgan}.

% Unfortunately, the previous text GANs are better doing sentence generation, while the fake data for taxonomy entrance evaluation are all concepts with fewer words than sentences.
% Since the semantic of a word is harder to be handled by the generative net, so using the existing text GANs do not have a good effect on concept generating.
% So we propose GANTEE (Generative Adversarial Network for Taxonomy Entrance Evaluation).
% GANTEE treat the generative model as an reinforcement learning agent; the state is the generate tokens combine with the prior information of anchor concepts, and the action is the next token to be generated.
% Rollout process \cite{yu2017seqgan} is proposed to alleviate the problem of gradient passing back, we regard that reward of rollout only are not enough for ``isA'' relation generating.
% So we take the rollout process as an short-term reward of the generating process, and propose another discriminator, which we called hyper discriminator, to detect whether the generated texts have a hypernym relation with the input anchor concept as an long-term reward.

% In the experiments, we benchmark the taxonomy entrance evaluation task on three real-world taxonomies in two different langauge, English and Chinese.
% We compare our method with other State-Of-Art methods to prove its effectiveness and efficiency.
% We make new State-Of-Art score by improve the hit@1 from \red{xxx} to \red{xxx}, MR from \red{xxx} to \red{xxx} and MRR from \red{xxx} to \red{xxx}.
% Then we also conduct experiments on traditional taxonomy expansion task, and GANTEE is still outperforms the baselines by a large margin on all three datasets.
% Finally, entensive experiments have been conducted to study how the parameters effect the result of GANTEE, and provide an effective tuning schemes for the following researchers who use our method in the future.

% \subsubsection{Contribution.}
% To summarize, our major contributions include: 
% (1): a more realistic task called taxonomy entrance evaluation which judge whether an query concept should be added into an existing taxonomy or not;
% (2): an novel, effective and PnP method called GANTEE to generating graph-level negative samples which boost the performance and the efficient for both traditional taxonomy expansion task and taxonomy entrance evaluation task.
% (3): extensive experiments that verify the effectiveness of GANTEE on three datasets in two language, and an effective tuning method was propose by the experiment.




==> 01_Introduction.1.tex <==
Taxonomy is formulated as directed acyclic graphs or trees, which consist of \emph{hyponym-hypernym} relations between concepts.
One concept is a hypernym of another concept if the meaning of the former covers the latter\cite{sang2007extracting}.
A well-constructed taxonomy can assist various downstream tasks, including web content tagging \cite{liu2020giant,liu2019tencent_taxonomy,peng2019RCNN4taxonomy}, personalized recommendation \cite{karamanolakis2020txtract, huang2019taxonomy, zhang2014taxonomy}, query understanding  \cite{yang2020co, hua2016understand} and so on. 


\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{introduction.png}
    \caption{An example of the new framework of taxonomy expansion task combined with the Taxonomy Entrance Evaluation task}
    \label{fig:introduction}
    \vspace{-5mm}
\end{figure}

Manually constructing and maintaining a taxonomy is labor-intensive, expensive, and time-consuming.
So the task of automated taxonomy expansion is hence proposed \cite{jurgens2016semeval},  which aims to automatically assign an existing concept (anchor concept) as a hypernym concept to the newly input concept (query concept).
The mainstream taxonomy expansion methods tend to use the self-supervised method to generate data from the existing taxonomy \cite{shen2020taxoexpan, yu2020steam, wang2021enquire, zhang2021taxonomy, mao2020octet, ma2021hyperexpan, wang2022qen}.
The accuracy of the automatic-annotated data is highly guaranteed, and the cost of both time and expense is much lower than previous methods.

\red{
However, these traditional taxonomy expansion methods only focus on calculate the similarity between each anchor concept to the query concept\cite{shen2020taxoexpan, yu2020steam, zhang2021taxonomy, wang2021enquire, wang2022qen}, and ignore the problem of whether the query concept should be added to the existing taxonomy at all.
These two tasks sound similar, but we consider they are different.
As we show in Figure \ref{fig:introduction}, when input ``The Eiffel Tower'' and ``Coconut Cake'' to the taxonomy of ``Computer Science'', previous methods will only calculate the similarity between the query concept to each of the anchor concept.
However, the similarity between anchor concept and unknown query concept are greatly determined by the initial representation of the query concept, and learning a good representation for all query concepts may be a huge expense since there are unlimited potential query concepts in real-scenrios.

without specific training, the similarity between unknown query concept and existing anchor concept are random, so even the input query concepts are noisy, the traditional taxonomy expansion model will probabily calculate a high similarity to it.
As in the real scenario, the query concepts are often noisy, as far as we know, none of the previous researches have studied such questions before, most of the researches just build self-supervised datasets which ignore it at all.
The consequence of ignoring such problem will cost another large labor-intensive expense to manually denoise the query concepts before the taxonomy expansion, since the taxonomy expansion model do not have the ability to distinguish the noisy. 

}

In this paper, we propose a new task, called taxonomy enterance evaluation, together with a corresponding method called Generative Adversarial Network for Taxonomy Enterance Evaluation (GANTEE).
Before the taxonomy expansion, we use GANTEE to evaluate whether a query concept should be added to the existing taxonomy.
And then the existing taxonomy evaluation methods are used to assign an anchor concept to the query concept.
The reasons why we introduce GANTEE are listed as follows:
\begin{itemize}
    \item GANTEE will make the model have a strong ability to distinguish the noisy query concepts.
    \item When the number of query concepts is large, the denoise method will best increase the efficiency of the whole process.
\end{itemize}

A pre-trained auto-regressive generative model is used in GANTEE to introduce the outside information to alleviate the above problems.
Beyond that, a pure auto-regressive is mainly used to generate sentence-level text, and the semantic of concept, which is word-level text, is hard to be captured.
So the extra supervised signal is needed to guarantee the generated text is a concept that has a hyponym relation to the given anchor query.

To this end, we use Generative Adversarial Network(GAN) \cite{goodfellow2014generative} to alleviate the above problem.
Specifically, in GAN a discriminative net $\mathcal{D}$ learns to tell the fake data apart from the real data, and the generative net $\mathcal{G}$ learns to confuse $\mathcal{D}$ by generating fake data which has similar distribution with the real data.
We take the generative model as a reinforcement learning agent; the state is the generated tokens combined with the prior information of anchor concepts, and the action is the next token to be generated.
The generated texts are expected to be a fake query concept which is a hyponym to the given anchor concept, but a question proposed by the previous research\cite{guo2018leakgan} that when the discriminator is too strict, the effective gradient won't be calculated, so we use a loose rollout discriminator and a strict hyper discriminator to provide supervised generative signal during the generating process.
Rollout process \cite{yu2017seqgan} is proposed to alleviate the problem of gradient passing back, which is used to guarantee that the generated text is a concept during the generating process.
A hyper discriminator is used to detect whether the generated query concept has a ``hyponym'' relation to the given anchor concept after the generating process.

In the experiments, we benchmark the taxonomy entrance evaluation task on three real-world taxonomies in two different languages, English and Chinese.
We make new State-Of-Art score in the experiments by improve the hit@1 from \red{xxx} to \red{xxx}, MR from \red{xxx} to \red{xxx} and MRR from \red{xxx} to \red{xxx}.
Then we test the efficiency of our method, and GANTEE still outperforms the baselines by a large margin on all three datasets.
Finally, extensive experiments have been conducted to study how the parameters affect the result of GANTEE, and provide an effective tuning scheme for the following researchers who will use our method in the future.

\subsubsection{Contribution.}
To summarize, our major contributions include: 
(1): a more realistic task called taxonomy entrance evaluation which judges whether a query concept should be added to an existing taxonomy or not;
(2): a novel, effective, and PnP method called GANTEE to generate graph-level negative samples which boosts the performance and the efficiency for both traditional taxonomy expansion tasks and taxonomy enterance evaluation tasks.
(3): extensive experiments that verify the effectiveness of GANTEE on three datasets in two languages, and an effective tuning method was proposed by the experiment.




==> 01_Introduction.2.tex <==
Taxonomy is formulated as directed acyclic graphs or trees, which consist of \emph{hyponym-hypernym} relations between concepts.
One concept is a hypernym of another concept if the meaning of the former covers the latter\cite{sang2007extracting}.
A well-constructed taxonomy can assist various downstream tasks, including web content tagging \cite{liu2020giant,liu2019tencent_taxonomy,peng2019RCNN4taxonomy}, personalized recommendation \cite{karamanolakis2020txtract, huang2019taxonomy}, query understanding  \cite{yang2020co} and so on. 

Manually constructing and maintaining a taxonomy is labor-intensive, expensive, and time-consuming.
So the task of automated taxonomy expansion is hence proposed \cite{jurgens2016semeval}, which aims to automatically assign an existing concept (anchor concept) as a hypernym concept to the newly input concept (query concept).
The mainstream taxonomy expansion methods tend to use the self-supervised method to generate data from the existing taxonomy \cite{shen2020taxoexpan, yu2020steam, wang2021enquire, zhang2021taxonomy, mao2020octet, ma2021hyperexpan, wang2022qen}.
The model will learn from the existing hypernym-hyponym relation, and  to assign anchor concepts to the new query concepts.
These models achieve great success in saving a lot of time from automated taxonomy construction and maintenance.

However, we argue that the assumption made by the previous taxonomy expansion researches that \emph{the query concepts are most clean} is not true in the real-scenarios.
We observe that the number of query concepts in real-scenarios are much larger than the number in the experiments of previous researches, and \emph{most query concepts are noisy}, which means they shouldn't be added to the existing taxonomy.
% We observe that huge amount of noisy query concepts are expected to be added to the existing taxonomy in the industry application, which make the amount of query concepts much larger than the experiment setting in the previous researches.
Tens of thousands of concepts are involved in the experiments of previous researches\cite{ zhang2021taxonomy, ma2021hyperexpan, wang2022qen}, and there are millions of new concepts expected to be added in Taobao taxonomy, which is the largest Chinese shopping platform, in a single time \cite{jiang2019towards}, and each year there will be billions of new concepts generated in Meituan online application \cite{cheng2022learning}, which is a leading Chinese e-commerce platform for ordering take-outs, and only thousands of them are finally added in the existing taxonomy.

The large amount of noisy concepts will greatly slow the efficiency and effectiveness of the previous methods.
These methods rely heavily on good concept representations, which can judge the hypernym-hyponym relationships of concepts through the similarity between representations.
Even with only tens of thousands of concepts in their experiments, the previous methods also spent a lot of time training the model to get a representation for each concept that satisfies the above condition\cite{yu2020steam, zhang2021taxonomy, wang2021enquire}.
The time expense of such progress will be unacceptable when the data scale increases from tens of thousands to billions.
We summarize the challenges of facing such large amount of noisy concepts and list as follows:
\begin{itemize}
    \item Large amount of concepts will consume huge amount of time in learning representation for every concept
    \item Even with a good representation, a large number of noisy query concepts is still a huge challenge to current taxonomy expansion models which do not even consider the problem of noisy concepts.
\end{itemize}


In this paper, we propose a plugin task called taxonomy enterance evaluation.
The taxonomy enterance evaluation aims at scoring the query concept to indicate whether this concept should be added to the existing taxonomy in an efficient way, the noisy concept is expected to get a low score, while the real concept is expected to be scored high.
The input will meet the assumption of taxonomy expansion task when low-score concepts are all excluded, the efficiency and effectiveness of taxonomy expansion will hence increase greatly.

We model the taxonomy enterance evaluation as a binary classification task, and obtain the representations of concepts by pretrained language models (PLMs).
With the rapid development of PLM, it has achieved a great success in the field of text understanding \cite{devlin2018bert, yang2019xlnet}.
With representation of every word is pretrained in PLM, it will quickly output the representation of whole text.
In order to efficiently get the representation of the concept, many works use language models to quickly obtain the representation through the textual information of the concept \cite{cheng2022learning, takeoka2021low}.
Although the language model has a limited ability in representing conceptual text, classifer will have strong discriminative ability with a large amount of high quality training data.
To ensure the quality of the training data, large amount of deceptive negative data and fedility positive data are needed, and simply sampling from existing Taxonomy is not enough.


Here, together with the taxonomy enterance evaluation task, we propose a corresponding method called \textbf{G}enerative \textbf{A}dversarial \textbf{N}etwork for \textbf{T}axonomy \textbf{E}nterance \textbf{E}valuation (GANTEE).
The discriminative model $\mathcal{D}$ in Generative Adversarial Network learns to give supervised signals of telling the generated text apart from the text in real query concept, and the generative model $\mathcal{G}$ learns to confuse $\mathcal{D}$ by generating text which has a deceptively ``hyponym'' relation to the given anchor concept.
The generated texts are expected to be a fake query concept which is a hyponym to the given anchor concept, but a question proposed by the previous research\cite{guo2018leakgan} that when the discriminator is too strict, the effective gradient won't be calculated, so we use a loose rollout discriminator and a strict hyper discriminator to provide supervised signal during the generating process.
Rollout discriminator is proposed to alleviate the problem of gradient passing back during the rollout process \cite{yu2017seqgan}, which is a process proposed to get the reward of unfinished text.
A hyper discriminator is used to detect whether the generated text has a ``hyponym'' relation to the given anchor concept after the generating process.

In the experiments, we benchmark the taxonomy entrance evaluation task on three real-world taxonomies in two different languages, English and Chinese.
We make new State-Of-Art score in the experiments by improve the hit@1 from \red{xxx} to \red{xxx}, MR from \red{xxx} to \red{xxx} and MRR from \red{xxx} to \red{xxx}.
Then we test the efficiency of our method, and GANTEE still outperforms the baselines by a large margin on all three datasets.
Finally, extensive experiments have been conducted to study how the parameters affect the result of GANTEE, and provide an effective tuning scheme for the following researchers who will use our method in the future.

\subsubsection{Contribution.}
To summarize, our major contributions include: 
(1): a more realistic task called taxonomy entrance evaluation which judge whether a query concept should be added to an existing taxonomy in an efficient way;
(2): a novel, effective method called GANTEE to generate confusing negative and fidelity positive data which boosts the performance and the efficiency for both traditional taxonomy expansion tasks and taxonomy enterance evaluation tasks.
(3): extensive experiments that verify the effectiveness of GANTEE on three datasets in two languages, and an effective tuning method was proposed by the experiment.

==> 01_Introduction.3.tex <==
Taxonomy is formulated as directed acyclic graphs or trees, which consist of \emph{hyponym-hypernym} relations between concepts.
One concept is a hypernym of another concept if the meaning of the former covers the latter \cite{sang2007extracting}.
A well-constructed taxonomy can assist various downstream tasks, including web content tagging \cite{liu2020giant,liu2019tencent_taxonomy,peng2019RCNN4taxonomy}, personalized recommendation \cite{karamanolakis2020txtract, huang2019taxonomy}, query understanding  \cite{yang2020co} and so on. 

Manually constructing and maintaining a taxonomy is labor-intensive and time-consuming.
For example, there are millions of new concepts expected to be added in Taobao taxonomy, which is the largest Chinese shopping platform, in a single time \cite{jiang2019towards}.
So the task of automated taxonomy expansion is proposed \cite{jurgens2016semeval}, which aims to automatically assign an existing concept (anchor concept) as a hypernym concept to the newly input concept (query concept).
The mainstream taxonomy expansion methods assume that most query concepts are clean.
They tend to learn from the hypernym-hyponym relation in the existing taxonomy, and assign anchor concepts to all query concepts \cite{shen2020taxoexpan, yu2020steam, wang2021enquire, zhang2021taxonomy, mao2020octet, ma2021hyperexpan, wang2022qen}.
These models achieve great success in saving a lot of time from labor annotation in taxonomy construction and maintenance.

However, we argue that there are two main differences between the previous studies and real-scenarios. 
\textbf{First}, only tens of thousands of query concepts were covered in the experiments of previous taxonomy expansion studies, which is far from the real-scenarios.
\textbf{Second}, the assumption made by the previous studies that most query concepts are clean is not true in the real-scenarios.
For instance, there have billions of new query concepts generated in Meituan online application \cite{cheng2022learning}, which is a leading Chinese e-commerce platform for ordering take-outs, and only thousands of them are clean and being added to the existing taxonomy.
Even with only tens of thousands of concepts in their experiments, it still take the previous methods a lot of time during the training and the predicting stage \cite{yu2020steam, zhang2021taxonomy, wang2021enquire}.
Because most of the previous methods rely heavily on concept representation techniques, these techniques use vector to represent conceptual features instead of text.
The representations of the concepts are expected to denote the hypernym-hyponym relationships based on the vectorized similarity.
And the time expense of learning a good representation will be unacceptable when the data scale increases from tens of thousands to billions during the predicting stage in real-scenarios.
One step more, even with a good representation, a large number of noisy query concepts is still a huge challenge to current taxonomy expansion models which do not even consider the problem of noisy concepts.

In this paper, we propose a plugin task called taxonomy enterance evaluation to alleviate the above problems, and a corresponding method called \textbf{G}enerative \textbf{A}dversarial \textbf{N}etwork for \textbf{T}axonomy \textbf{E}nterance \textbf{E}valuation (GANTEE).
From the case of Meituan, we find that most of query concepts are noisy in real-scenarios.
So the task of taxonomy enterance evaluation aims at excluding noisy query concepts before taxonomy expansion, leaving clean query concepts to increase the efficiency of taxonomy expansion.
Intuitively, taxonomy enterance evaluation task can be modeled as a binary classification task, but such modeling brings two challenges.
\begin{itemize}
    \item Large amount of high quality positive and negative data are needed to do the training.
    \item The efficiency of this task should be high enough to reduce the time expense of whole automated taxonomy construction and maintenance task.
\end{itemize}

The existing hypernym-hyponym can be used as training data, which can be on solution to the challenge of the training data.
And with the rapid growth of pretrained language models (PLMs), one can quickly fetch the representation of concept based on the text of concept since PLMs have pretrained every token of the text, which can be one solution to the challenge of the efficiency.
However, simply sampled from the existing taxonomy only produce weak training data, and PLMs have limited ability in representing hypernym-hyponym relation based on its pretrained representation.
Combine the above methods, GANTEE will do much better not only taxonomy enterance evaluation, but also taxonomy expansion.

GANTEE use Generative Adversarial Network (GAN) to produce deceptively negative data and fidelity positive data with theoretically infinite number.
PLMs are used during the adversarial process to enforce the discriminative model $\mathcal{D}$ to distinguish the hypernym-hyponym relationships based on the representation of PLMs, rather than relying on similarity as in the previous method.
And designed discriminative model $\mathcal{D}$ learns to give supervised signals of telling the generated text apart from the text in real query concept, and the generative model $\mathcal{G}$ learns to confuse $\mathcal{D}$ by generating text which has a deceptively ``hyponym'' relation to the given text of an anchor concept.
The generated texts are expected to be a fake query concept which is a hyponym to the given anchor concept, but a question proposed by the previous research\cite{guo2018leakgan} that when the discriminator is too strict, the effective gradient won't be calculated, so we use a loose rollout discriminator and a strict hyper discriminator to provide supervised signal during the generating process.
Rollout discriminator is proposed to alleviate the problem of gradient passing back during the rollout process \cite{yu2017seqgan}, which is a process proposed to get the reward of unfinished text.
A hyper discriminator is used to detect whether the generated text has a ``hyponym'' relation to the given anchor concept after the generating process.

In the experiments, we benchmark the taxonomy entrance evaluation task on three real-world taxonomies in two different languages, English and Chinese.
We make new State-Of-Art score in the experiments by improve the hit@1 from \red{xxx} to \red{xxx}, MR from \red{xxx} to \red{xxx} and MRR from \red{xxx} to \red{xxx}.
Then we test the efficiency of our method, and GANTEE still outperforms the baselines by a large margin on all three datasets.
Finally, extensive experiments have been conducted to study how the parameters affect the result of GANTEE, and provide an effective tuning scheme for the following researchers who will use our method in the future.

\subsubsection{Contribution.}
To summarize, our major contributions include: 
(1): a more realistic task called taxonomy entrance evaluation which judge whether a query concept should be added to an existing taxonomy in an efficient way;
(2): a novel, effective method called GANTEE to generate confusing negative and fidelity positive data which boosts the performance and the efficiency for both traditional taxonomy expansion tasks and taxonomy enterance evaluation tasks.
(3): extensive experiments that verify the effectiveness of GANTEE on three datasets in two languages, and an effective tuning method was proposed by the experiment.

==> 01_Introduction.4.tex <==
Taxonomy is formulated as directed acyclic graphs or trees, which consist of \emph{hyponym-hypernym} relations between concepts.
One concept is a hypernym of another concept if the meaning of the former covers the latter \cite{sang2007extracting}.
A well-constructed taxonomy assist various downstream tasks, including web content tagging \cite{liu2020giant,liu2019tencent_taxonomy,peng2019RCNN4taxonomy}, personalized recommendation \cite{karamanolakis2020txtract, huang2019taxonomy}, query understanding  \cite{yang2020co} and so on. 

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{intro.pdf}
    \caption{An example of the GANTEE framework. This framework is implemented as a plugin before taxonomy expansion. The demand of generating high-quality data and taxonomy enterance evaluation are formulated as a generative adversarial network in GANTEE.}
    \label{fig:introduction}
    \vspace{-5mm}
\end{figure}

Manually constructing and maintaining a taxonomy is labor-intensive and time-consuming.
For example, there are millions of new concepts expected to be added in Taobao taxonomy, which is the largest Chinese shopping platform, in a single time \cite{jiang2019towards}.
So the task of automated taxonomy expansion is proposed \cite{jurgens2016semeval}, which aims to automatically assign an existing concept (anchor concept) as a hypernym concept to the newly input concept (query concept).
\red{
The mainstream taxonomy expansion methods assume that most query concepts are clean.
These methods model taxonomy expansion task as binary classification, sampling two concepts connected by the existing edges in the taxonomy as positive training data, and random two concepts as negative training data.
To improve the performance of the models, they spent a lot of time on learning representations for each concepts.
And they use sampled training data based-on learned representation to assign anchor concepts to all query concepts \cite{shen2020taxoexpan, yu2020steam, wang2021enquire, zhang2021taxonomy, mao2020octet, ma2021hyperexpan, wang2022qen}.
}
These models achieve great success in saving a lot of time from labor annotation in taxonomy construction and maintenance.

However, we argue that there are two main gaps between the previous studies and real-scenarios. 
\textbf{First}, the assumption made by the previous studies that most query concepts are clean is not true in the real-scenarios.
For instance, there have billions of new query generated in an ordering take-outs online application \cite{cheng2022learning} in five months time, and only thousands of them are clean and being added to the existing taxonomy.
Since the previous methods spent a lot of time on representation learning, large amount of noisy query concepts will greatly slow the \red{predicting speed}.
\textbf{Second}, there is a large gap on the semantic between the hypernym-hyponym relationships in the existing taxonomy and in real-scenrios.
Many companies invite experts to build a taxonomy consisting of thousands of concepts and expect taxonomy expansion methods to expand this taxonomy into the level of millions or even billions of concepts.
Only use concepts in the existing taxonomy as training data limits the ability of the model in finding new hypernym-hyponym relationship in real-scenrios.
So the effectiveness of the previous taxonomy expansion methods will be greatly reduced in the real-scenarios.



In this paper, we propose a plugin task called taxonomy enterance evaluation to alleviate the first problem.
This task aims at excluding noisy query concepts before taxonomy expansion in an efficient way.
At the same time, more high-quality data are required during the model training stage in taxonomy expansion task to alleviate the second problem.
Combine these two demands, we propose a corresponding plugin framework called \textbf{G}enerative \textbf{A}dversarial \textbf{N}etwork for \textbf{T}axonomy \textbf{E}nterance \textbf{E}valuation (GANTEE).

The example of GANTEE framework is shown in Figure \ref{fig:introduction}.
We model the first and second problems as an generative adversarial task.
The discriminative model is used to identify the noisy query concepts (generated query concepts) from the real query concepts.
And the generative model is used to generate fake query concepts which has similar semantic to the real query concepts to confuse the discriminative model.
The generated data is also used to train the taxonomy expansion model, since the generated positive data are fidelity and unseen to the existing taxonomy, and the generated negative data are more deceptive than random sampling methods, which can further improve the judging ability of the taxonomy expansion models.

% To ensure the efficiency, we use pretrained language models (PLMs) to get the representation for every concept based on the textual feature of the text.
% This is a trade off between the efficiency with the effectiveness, the PLMs has limited ability in representing conceptual text, but with vast of training data generated by the generative model, the shortage of the representation is compensated.

To ensure the efficiency, we use pre-trained language models (PLM) to obtain a representation of each concept based on the textual features of the concept.
This approach is actually a trade-off between efficiency and effectiveness.
PLMs can obtain a representation from the textual features of concepts in a very short time, the reason why previous works do not use PLMs is because PLMs have limited ability in representing the fine-grained semantics based on conceptual text.
We compensate for the lack of PLMs representation capability by reducing the denoising problem into an coarse-grained evaluation problem and generating large amount of high-quality training data by the generative model.
% We reduce the denoising problem to an coarse-grained evaluation problem, and compensate for the lack of PLM representation capability by generating the large amount of high-quality training data generated in the model.

% PLMs can obtain a representation from the textual features of concepts in a very short time, but the reason why previous works do not use PLMs is because PLMs have limited capability to represent the text of concepts.
% We compensate for the lack of PLMs representation capability by the large amount of high-quality training data generated in the generative model.

In the experiments, we benchmark the taxonomy entrance evaluation task on three real-world taxonomies in two different languages, English and Chinese.
We make new State-Of-Art score in the experiments by improve the hit@1 from \red{xxx} to \red{xxx}, MR from \red{xxx} to \red{xxx} and MRR from \red{xxx} to \red{xxx}.
Then we test the efficiency of our method, and GANTEE still outperforms the baselines by a large margin on all three datasets.
Finally, extensive experiments have been conducted to study how the parameters affect the result of GANTEE, and provide an effective tuning scheme for the following researchers who will use our method in the future.

\subsubsection{Contribution.}
To summarize, our major contributions include: 
(1): a more realistic task called taxonomy entrance evaluation which judge whether a query concept should be added to an existing taxonomy in an efficient way;
(2): a novel, effective method called GANTEE to generate confusing negative and fidelity positive data which boosts the performance and the efficiency for both traditional taxonomy expansion tasks and taxonomy enterance evaluation tasks.
(3): extensive experiments that verify the effectiveness of GANTEE on three datasets in two languages, and an effective tuning method was proposed by the experiment.

==> 01_Introduction.5.tex <==
Taxonomy is formulated as directed acyclic graphs or trees, which consist of \emph{hyponym-hypernym} relations between concepts.
One concept is a hypernym of another concept if the meaning of the former covers the latter \cite{sang2007extracting}.
A well-constructed taxonomy assist various downstream tasks, including web content tagging \cite{liu2020giant,liu2019tencent_taxonomy,peng2019RCNN4taxonomy}, personalized recommendation \cite{karamanolakis2020txtract, huang2019taxonomy}, query understanding  \cite{yang2020co} and so on. 

\begin{figure*}
    \centering
    \includegraphics[width=0.8\linewidth]{intro.png}
    \caption{An example of the GANTEE framework. This framework is implemented as a plugin before taxonomy expansion. The demand of generating high-quality data and taxonomy enterance evaluation are formulated as a generative adversarial network in GANTEE.}
    \label{fig:introduction}
    \vspace{-5mm}
\end{figure*}

Manually maintaining a taxonomy is labor-intensive and time-consuming.
For example, millions of new concepts are expected to be added to the taxonomy of one of the largest shopping platforms in the world each month \cite{jiang2019towards}.
So the task of automated taxonomy expansion is proposed \cite{jurgens2016semeval}, which aims to automatically assign an existing concept (anchor concept) as a hypernym concept to the newly input concept (query concept).
These models achieve great success in saving a lot of time from labor annotation in taxonomy maintenance.
%The prevailing taxonomy expansion methods assume that most query concepts are clean.
These methods predict the hypernym-hyponym relationships mainly based on the representation similarity, so they sample the training data based on the existing taxonomy to learn good representations for each concept. 

However, we argue that these methods cannot be applied to real applications due to two drawbacks. 
\textbf{First}, these methods suffer from low effectiveness in real applications due to limited ability to represent semantics of concepts. Only sampling from existing taxonomy provides limited data to train representations for zero-shot concepts, where most of the query concepts are zero-shot concepts.
%there is a few-shot problem in real scenarios that only sampling from the existing taxonomy does not provide enough diverse data to train the model which can mine the hypernym-hyponym relationships in real scenarios.
Previous work shows that xx~\cite{cheng2022learning}.
%Since the data in real scenarios is usually thousands of times the size of the concept in the existing taxonomy, only sampling from the existing taxonomy will greatly harm the effectiveness of the previous taxonomy expansion methods in the real scenarios.
\textbf{Second}, these methods suffer from low efficiency in real applications because most of the query concepts are noisy. %Previous methods assume that the query concepts are clean.
For instance, in a leading ordering take-outs online platform, only thousands of concepts out of billions of queries are finally added to their taxonomy\cite{cheng2022learning}.
Previous methods ignore the noisy concepts and waste a lot of time to find the anchor concept for noisy query concepts.
%A large number of noisy concepts will result in a huge time expense in learning a good representation during the predicting stage in taxonomy expansion.


In this paper, we propose a plugin framework called \textbf{G}enerative \textbf{A}dversarial \textbf{N}etwork for \textbf{T}axonomy \textbf{E}nterance \textbf{E}valuation (GANTEE) to boost both the effectiveness and efficiency of the taxonomy expansion methods in real-scenarios as is shown in Figure \ref{fig:introduction}.
To improve the effectiveness, GANTEE proposes a generative model to generate more high-quality training data, which are required to train the high-quality representation for taxonomy expansion. 
To improve the efficiency, GANTEE introduces a new task called taxonomy entrance evaluation, which removes the large amount of noisy query concepts before finding the suitable anchor concept for them.
Intuitively, the generative model and the taxonomy entrance evaluation model are two adversarial models which can improve each other. The generative model produces more fake samples which are similar to the real samples to confuse the discriminative model, and the taxonomy entrance evaluation model learns to generate high quality samples. Therefore, these two tasks can be formulated as a generative adversarial task\cite{goodfellow2014generative} to further improve their performance.

Specifically, in order to improve efficiency, the taxonomy entrance evaluation model is expected to be more light-weight than taxonomy expansion model. We introduce two mechanisms to ensure the efficiency of taxonomy entrance evaluation model. First, instead of determining where to extend the query concept, GANTEE introduce two easier tasks xx and xx to determine whether the query concept is a concept and whether the query concept should be added to the taxonomy.
Second, instead of training a new representation for emerging query concepts, we use pre-trained language models (PLMs) to directly obtain a representation of each concept based on the textual features of the concept. Although PLMs have limited ability in representing the fine-grained semantics based on conceptual text\cite{lauscher2019specializing}, the experimental results verify that PLMs are suitable to generate representation for xx and xx.



%This approach is a trade-off between efficiency and effectiveness.
%PLMs can obtain a representation from the textual features of concepts in a very short time\cite{devlin2018bert}, the reason why previous works do not use PLMs is that PLMs have limited ability in representing the fine-grained semantics based on conceptual text\cite{lauscher2019specializing}.
%We compensate for the lack of PLMs representation capability by reducing the denoising problem into a coarse-grained evaluation problem and generating a large amount of high-quality training data by the generative model.

In the experiments, we benchmark the taxonomy entrance evaluation task on three real-world taxonomies in two different languages, English and Chinese.
We make new State-Of-Art score in the experiments by improve the hit@1 from \red{xxx} to \red{xxx}, MR from \red{xxx} to \red{xxx} and MRR from \red{xxx} to \red{xxx}.
Then we test the efficiency of our method, and GANTEE still outperforms the baselines by a large margin on all three datasets.
Finally, extensive experiments have been conducted to study how the parameters affect the result of GANTEE, and provide an effective tuning scheme for the following researchers who will use our method in the future.

\subsubsection{Contribution.}
To summarize, our major contributions include: 
(1) a more realistic task called taxonomy entrance evaluation which judge whether a query concept should be added to an existing taxonomy in an efficient way;
(2) a novel, effective method called GANTEE to generate confusing negative and fidelity positive data which boosts the performance and the efficiency for both traditional taxonomy expansion tasks and taxonomy enterance evaluation tasks.
(3) extensive experiments that verify the effectiveness of GANTEE on three datasets in two languages, and an effective tuning method was proposed by the experiment.

==> 02_ProblemFormulation.tex <==
In this section, we first give the definitions of the preliminary concepts used in this paper, then formally define the taxonomy enterance evaluation task and traditional taxonomy expansion problems.

\subsection{Preliminaries} \label{sec:define}

\begin{myDef}
\textbf{(Taxonomy and Anchor Concept.)}
A taxonomy $\mathcal{T}=(\mathcal{C}_{\mathcal{A}}, \mathcal{E})$ is a directed acyclic graph.
Each node $c_q \in \mathcal{C}_{\mathcal{A}}$ denotes an anchor concept and each directed edge $\langle n_{q}^{p}, n_{q}^{c} \rangle \in \mathcal{E}$ represents the hyponymy relation between the parent (hypernym) concept $n^c_p$ and the child (hyponym) concept $n^c_q$.
\end{myDef}

\begin{myDef}
\textbf{(Query Concept.)}
Query concept is the concept prepared to be added into the existing taxonomy.
The set of query concepts is represented as $\mathcal{C}_{\mathcal{Q}} = \{c^1_q, c^2_q, \cdots, c^m_q\}$.
While the previous studies assume the query concepts can all be added into the existing taxonomy, we argue that would not be true in the real scenario, and we will discuss the detail of it in the Problem \ref{taxonomy enterance evaluation}.
\end{myDef}


\subsection{Problem Definition}


\begin{myproblem}
\label{taxonomy enterance evaluation}
\textbf{(Taxonomy Enterance Evaluation.)}
Given an existing taxonomy $\mathcal{T}^{0}=(\mathcal{C}^{0}_{\mathcal{A}}, \mathcal{E}^{0})$ and the set of query concepts $\mathcal{C}_{\mathcal{Q}}$,
the goal of taxonomy enterance evaluation task is to score a query concept $c_q \in \mathcal{C}_{\mathcal{Q}}$ of the existing taxonomy $\mathcal{T}^{0}$, and the score bigger than the threhold $\gamma$ are considered as the concepts should be added into the taxonomy and are taken into the following steps.
\end{myproblem}
Formally, we consider each query concept $c_q \in \mathcal{C}_{\mathcal{Q}}$ and the taxonomy $\mathcal{T}^{0}$ as two random variables.
The task of taxonomy enterance evaluation can be formulated as follows:

% \red{
% \begin{equation}
% \small
% \begin{aligned}
% \mathcal{C}^{*} &=\underset{\mathcal{C}}{\arg \max } \mathbf{P}(C\mid\mathcal{T}^{0} ; \Theta_1)\\
% &=\underset{\mathcal{C}}{\arg \max } \sum_{i=1}^{\left|\mathcal{C}\right|} \log \mathbf{P}\left(c_{i} \mid \mathbf{T}^{0}; \Theta_1\right).
% \end{aligned}
% \end{equation}
% }
\begin{equation}
    \mathcal{C}_\mathcal{Q}^*=\{c_q^i\}\ \forall c_q^i \ s.t.\ p(c_q^i|\mathcal{T}^{0};\Theta_1)>\gamma
\end{equation}
where $\Theta_1$ denotes model parameters, and the $\mathcal{C}_\mathcal{Q}^*$ are the clean query concepts we have found.
% \red{
% We then find the optimal query concepts set $\mathcal{C}^{*}$ larger than a minimized size to maximize the likelihood.
% }

\begin{myproblem}
\textbf{(Taxonomy Expansion.)}
Given an existing taxonomy $\mathcal{T}^{0}=(\mathcal{C}^{0}_{\mathcal{A}}, \mathcal{E}^{0})$, the set of clean query concepts $\mathcal{C}_\mathcal{Q}^*$, the goal of taxonomy expansion task is to attach every query concept $c_q \in \mathcal{C}_\mathcal{Q}^*$ to the existing taxonomy $\mathcal{T}^{0}$ and expand it to obtain an enriched taxonomy $\mathcal{T}^{*}=(\mathcal{C}^{0}_{\mathcal{A}} \cup  \mathcal{C}_\mathcal{Q}^*, \mathcal{E}^{0} \cup \mathcal{R})$, where $\mathcal{R}$ is a set of new hyponymy relations $\langle c_a, c_q \rangle$, $c_a \in \mathcal{C}^{0}_{\mathcal{A}}$, $c_q \in \mathcal{C}_\mathcal{Q}^*$.
\end{myproblem}

Formally, we consider each node $c_q^{i} \in \mathcal{C}^{0}_\mathcal{Q}$ as a random variable and the taxonomy $\mathcal{T}^{0}$ as a Bayesian network.
The probability of taxonomy $\mathcal{T}^{0}$ can be formulated as follows.
\begin{equation}
\small
\mathbf{P}(\mathcal{T} \mid \Theta)=\mathbf{P}(\mathcal{C}_\mathcal{Q} \mid \mathcal{T}^{0}; \Theta)=\prod_{i=1}^{|\mathcal{C}_\mathcal{Q}|} \mathbf{P}\left(c^{i}_q \mid p\left(c^{i}_q\right); \Theta\right).
\end{equation}
where $\Theta$ denotes model parameters, and $p\left(c_q^{i}\right)$ represents the parent concept(s) of $c_q^{i}$.
We then find the optimal taxonomy $\mathcal{T}^{*}$ by maximizing the likelihood.
\begin{equation}
\small
\begin{aligned}
\mathcal{T}^{*} &=\underset{\mathcal{T}}{\arg \max } \mathbf{P}(\mathcal{T} \mid \Theta) \\
&=\underset{\mathcal{T}}{\arg \max } \sum_{i=1}^{\left|\mathcal{C}^{0}_{\mathcal{A}} \cup  \mathcal{C}_\mathcal{Q}^*\right|} \log \mathbf{P}\left(c_{i} \mid p\left(c_{i}\right); \Theta\right).
\end{aligned}
\end{equation}

However, for every node in the existing taxonomy, all query concepts in $\mathcal{C}^*$ can be taken as candidates of hyponym, thus the potential search space is incredibly enormous.
We follow the previous studies \cite{manzoor2020expanding, shen2020taxoexpan, yu2020steam, zhang2021taxonomy, mao2020octet} address the above problem via an assumption that the input set of new concepts contains only one element (i.e., $|\mathcal{C}^*_\mathcal{Q}|=1$), and aims to find one single parent node in the existing taxonomy $\mathcal{T}^{0}$ of this new concept (i.e., $|\mathcal{R}|=1$).
As a result, we divide the above computationally intractable problem into the following set of $|C^*|$ tractable optimization problems:
$$c_a^{i*}=\underset{c_a^i\in \mathcal{C}^0_\mathcal{A}}{\arg\max}logP(c_q^j|c_a^i,\Theta),\space \forall j\text{ or }i\in \{1,2,\dots,|C_\mathcal{Q}^*|\},$$
where $c_a^{i*}$ is the parent node of a new concept $c_q^i\in \mathcal{C}_\mathcal{Q}$.





==> 03_Method.0.tex <==

GANTEE consists of a generator $G$ and two descriminators, which are hyper discriminator $D_H$ and rollout descriminator $D_R$. 
$G$ takes an anchor concept as input and generates the corresponding query concept. 
$D_H$ determines whether the given anchor concept is suitable for the generated query concept, and $D_R$ determines whether the generated text is a concept.

Specifically, in the predicting stage, when a new query concept is given, GANTEE first determine if it is a concept by $D_R$. 
Then GANTEE determine whether the given concept has a hypernym-hyponym relation to the root concept by $D_H$.
Finally, GANTEE output a confidence score of whehther the given query concept is suitable for this taxonomy.
% $D_H$ takes the root concept as the anchor concept, and therefore $D_H$ determines whether the given query concept is suitable for this taxonomy.


\subsection{The Generative Model for Query Concept Generating}
We use Transformer \cite{vaswani2017attention} as the generative model.
Transformer maps the input sequence $x_1,\dots,x_n$ into a sequence of hidden states $\mathbf{h_1},\dots,\mathbf{h_n}$.
Specificly, a Transformer block consist of stacked self-attention layers with residual connections.
Each self-attention layer receives $n$ embeddings $\{x_i\}^n_{i=1}$ corresponding to unique input tokens, and outputs $n$ embeddings $\{h_i\}^n_{i=1}$, preserving the input dimensions.
The $i$-th token is mapped via linear transformations to a key $k_i$, query $q_i$, and value $v_i$.
The $i$-th output of the self-attention layer is given by weighting the values $v_j$ by the normalized dot product between the query $q_i$ and other keys $k_j$:
\begin{equation}
    h_i=\sum^n_{j=1}softmax(\langle q_i,k_{j'}\rangle^n_{j'=1})_j\cdot v_j
\end{equation}

This allows the layer to assign ``credit'' by implicitly forming state-return associations via similarity of the query and key vectors (maximizing the dot product). 
It is worth noticing that most of the Transformer variants, such as BART \cite{lewis2019bart} or XLNet \cite{yang2019xlnet}, and the RNN variants, such as the Gated Recurrent Unit(GRU) \cite{cho2014gru} or Long-Short Term Memory network(LSTM) \cite{hochreiter1997lstm}, can be used as a generator in GANTEE.
But we use GPT-2 \cite{radford2019gpt2} in this paper to give the best experiment results.
GPT-2 modifies the transformer architecture with a causal self-attention mask to enable auto-regressive generation, it is known as the most famous auto-regressive model, which suits the task of fake query generation best.

\begin{figure*}
    \centering
    \includegraphics[width=1\linewidth]{intro.png}
    \caption{An example of the GANTEE framework. This framework is implemented as a plugin before taxonomy expansion. The demand of generating high-quality data and taxonomy entering evaluation are formulated as a generative adversarial network in GANTEE.}
    \label{fig:introduction}
    \vspace{-5mm}
\end{figure*}
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{Framework.png}
    \caption{The framework of GANTEE.
    The generator of the GANTEE is on the left, and the duel discriminator is on the right.
    The detail information of this framework is in Section \ref{03}}
    \label{fig:framework.png}
\end{figure}

\subsection{The Rollout Discriminative Model for Short Term Reward in Generating}
Rollout discriminative model is used to judge whether the generated text is a concept before the generating process finish.
Deep discriminative models such as deep neural network(DNN), convolutional neural network(CNN) and recurrent convolutional neural network(RCNN) have shown a high performance in complicated sequence classification tasks.
In this paper, we choose LSTM\cite{hochreiter1997lstm} as our rollout discriminator since it is a lightweight model which is easy to do the training and won't have a so strict discriminative ability to the generated text.
LSTM will take in the input embedding $\mathbf{x_1},\dots,\mathbf{x_t}$ and use purpose-built memory cells to calculate the hidden state for each step $\mathbf{h_0}, \mathbf{h_1} \dots, \mathbf{h_t}$.
\begin{equation}
    \begin{aligned}
    % &i_t=\sigma\left(W_{xi}\mathbf{x_t}+W_{hi}\mathbf{h_{t-1}}+W_{ci}\mathbf{c_{t-1}}+\mathbf{b_i}\right),\\
    % &f_t=\sigma\left(W_{xf}\mathbf{x_t}+W_{hf}\mathbf{h_{t-1}}+W_{cf}\mathbf{c_{t-1}}+\mathbf{b_f}\right),\\
    % &c_t=f_t c_{t-1}+i_t tanh(W_{xc}\mathbf{x_t}+W_{hc}\mathbf{h_{t-1}}+\mathbf{b_{c}}),\\
    % &o_t=\sigma\left(W_{xo}\mathbf{x_t}+W_{ho}\mathbf{h_{t-1}}+W_{co}c_t+\mathbf{b_o}\right),\\
    % &h_t=o_t tanh(c_t).
    h_t = lstm(x_1,\cdots,x_t)
    \end{aligned}
\end{equation}
Where $\sigma$ is the logistic sigmoid function, and $i,\ f,\ o\text{ and }c$ are the input gate, forget gate, output gate and cell vectors, all of which are the same size as the hidden vector $h$.
We take the final hidden state $h_t$ and inject it into a linear layer to calculate the reward of the generated text:
\begin{equation}
    r_r = W_r \cdot \mathbf{h_t}+\mathbf{b_r}
\end{equation}
Where $W_r$ and $\mathbf{b_r}$ are the parameters in linear layer, the $r_r$ is the probability of the generated text is a concept.
% In this paper, we choose Bert\cite{devlin2018bert} as our discriminator as Bert has been shown of great effectiveness in Dependency Judgment task\cite{shi2019next}, which is good at understanding the hypernym relation .
% Most discriminative models can only perform classification well for an entire sequence rather than the unfinished one. 
% In this paper, we also focus on the situation where the discriminator predicts the probability that a finished sequence is real.
% We first represent an input sequence $x_1, \dots, x_t$ with the prior anchor concept $c_0:\{x^{c_0}_1,\dots,x^{c_0}_t\}$ as:
% $$\mathbb{E}_{1:t}=x^{c_0}_1\oplus \dots\oplus x^{c_0}_t\oplus x_1\oplus x_2\oplus \dots \oplus x_t$$
% where $x_i\in\mathbb{R}^k$ is the $k$-dimensional token embedding and $\oplus$ is the concatenation operator to build the matrix $\mathbb{E_{1:T}}\in \mathbb{R}^{T\times k}$.

% The optimization target is to minimize the cross entropy between the ground truth label and the predicted probability as formulated in Eq. \ref{eqt:object fucntion}.

\subsection{The Hyper Discriminative Model for Long Term Reward in Generating}
Hyper discriminative model is used to judge whether the generated concept has a hypernym relation to the prior concept after the generating process finish.
Such discriminative model offer a long term reward for the generating process, to better guide the direction of the generation.
The existing models for taxonomy expansion can be used as the hyper discriminative model, which has the ability of detect whether there is an hypernym relation between two concepts.

However, such model rely heavily on the vector representation of the concepts, many researches such as STEAM\cite{yu2020steam} or TMN\cite{wang2021enquire} use external information to get better representations for the concepts, and that would be really time consuming for the generating process, since each time the generative model produce a new concept, it will take time to get its detailed information and get its vector representation.

Instead, we use Bert\cite{devlin2018bert} to retrieval the representation of concepts since it shows its ability in Dependency Judgement task\cite{shi2019next}, which is also good at understanding the hypernym (hyponym) relation between two concepts.
We concatnate the position embedding proposed by the TaxoExpan\cite{shen2020taxoexpan} to the Bert representation, and put them into a linear layer to get the final predict result.

Specificly, we get the representation of the concept by the Bert in the following format:
\begin{equation}
\small
\begin{aligned}
    &x_{a}=Bert(x^{c_0}_1,\dots,x^{c_0}_t)[1]\\
    &x_{q}=Bert(x_1,\dots,x_t)[1]
\end{aligned}
\end{equation}
Then, we concatnate the position embedding to the representation of the anchor concept and the query concept, and put them into a linear layer:
\begin{equation}
\small
    r_h=W_h\cdot(x_{a}+p_{a}+x_{q}+p_{q}) + b_h
\end{equation}
Where $W_h$ and $\mathbf{b_h}$ are the parameters in linear layer, $p_{a}$ and $p_q$ are the position embedding, and the $r_h$ is the probability of the hypernym relation between the generated query concept and the anchor concept. 


\subsection{Policy Gradient for GANTEE}
GANTEE use a GAN model to combine the training data generating task and noisy query denoise task.
It need generative model to generate conceptual text, and use discriminative model to offer supervised signals to the generative model, but naive GAN is used for continuous data but not for discrete tokens.
The previous researchers \cite{bachman2015data, bahdanau2016actor, yu2017seqgan} propose to consider the text generation procedure as a sequential decision making process.
The objective function of such generative models is formulated to generate a sequence from the start state $s_0$ to maximize its expected end reward via policy gradient algorithms \cite{sutton1999policy}:
\begin{equation}
    \begin{aligned}
        J(\theta)&=\mathbb{E}[R_T|s_0=c_a;\theta]\\&=\sum_{y_1\in Y}G_\theta(y_1|s_0=c_a)\cdot Q^{G_\theta}_{D_\phi}(s_0=c_a, y_1),
    \end{aligned}
\end{equation}
where $J(\theta)$ is the object function, $R_T$ is the reward for a complete concept which has hypernym relation to the given concept $c_a$.
Note that the reward is from the hyper discriminator $D_{\phi H}$ and rollout discriminator $D_{\phi R}$, which we will discuss later.
$G_\theta$ is the generative model, and $Q^{G_\theta}_{D_\phi}(s,a)$ is the action-value function of a sequence, which is calculated in the following format:
\begin{equation}
    Q^{G_\theta}_{D_\phi}(a=y_t, s=Y_{1:t-1}, s_0) = D_{\phi}(s_0, Y_{1:t-1})
\end{equation}
Since the reward getting from an unfinished sequence often have large bias from the finished one, Monte Carlo search is used to sample the unknown last $T-t$ tokens\cite{yu2017seqgan}:
\begin{equation}
        \{Y^1_{1:T},\dots,Y^N_{1:T}\}=MC^{G_\theta}\left(Y_{1:t};N\right)
\end{equation}

Since a severe gradient vanishing occurs when discriminator $D_\phi$ is too strict.
So we use rollout discriminator $D_{\phi R}$ to calculate the expected reward based on Monte Carlo search during the genertive process for short-term reward, and use hyper discriminator $D_{\phi H}$ to calculate the reward when the generating is done for long-term reward. 
And the action-value function is hence transformed into the following format:
\begin{equation}
    \small
    \begin{aligned}
    &Q^{G_\theta}_{D_\phi}(a=y_t, s=Y_{1:t-1}, s_0) = \\
    &\begin{cases}
    \frac{1}{N}\sum^N_{n=1}D_{\phi R}(s_0, Y_{1:t-1}), Y^n_{1:T}\in MC^{G_\theta}\left(Y_{1:t};N\right)& \text{for }t<T\\
    D_{\phi H}(Y_{1:t}, s_0)& \text{for }t=T
    \end{cases}
    \end{aligned}
\end{equation}

Once we have a set of more realistic generated sequences, we will re-train the discriminator model as follows:
\begin{equation}
    \label{eqt:object fucntion}
    \min_{\phi}-\mathbb{E}_{Y~p_data}[\log D_\phi(Y)]-\mathbb{E}_{Y~G_\theta}[log(1-D_\phi(Y))]
\end{equation}

In summary, we will pre-train the generator and the discriminator before the adversarial process begin.
And after the pre-training stage, the generator and discriminator are trained alternatively.
As the generator gets progressed via training on g-steps updates, the discriminator needs to be re-trained periodically to keeps a good pace with the generator.
When training the discriminator, positive examples are sampled from the existing taxonomy $\mathcal{T}^{0}$ based on the hypernym relation $\mathcal{R}$, whereas negative examples are generated from our generator.
To ensure the learning process doing well, we use both of the fake query concepts together with the pure noisy text to as the negative query concepts to inject into the training process, and the number of negative query concepts we use is the same as the size of positive query concepts.

% \subsection{Improvement in the Higher-Quality Training Data Generating}
% Here we propose three extra methods to further improve the 
% To improve the effectiveness of taxonomy expansion, here we propose three extra methods which can generate training samples with higher-quality.

% First, we propose a positive and negative given generating methods

% Second, we propose to use Graph Convolutional Network to represent the whole taxonomy, and us
% Second, we propose to use Graph Convolutional Network to representation the whole taxonomy, and use such 

==> 05_RelatedWork.0.tex <==


\subsection{Taxonomy Expansion}
In taxonomy expansion task, an existing taxonomy such as WordNet\cite{miller1995wordnet} or Probase\cite{wu2012probase,chen2019cnprobase} is provided as both the guidance and the base for adding new terms. 
Aly \emph{et al.}\cite{aly2019every} adopt hyperbolic embedding to capture hierarchical lexical-semantic relations.
Fauceglia \emph{et al.}\cite{fauceglia2019automatic} use a hybrid method to combine linguistic patterns, semantic web, and neural network for taxonomy expansion.
Manzoor \emph{et al.}\cite{manzoor2020expanding} model the implicit edge semantics to score the hyponymy relevance between node pairs. 
However, the above methods fail to exploit the structural information of the existing taxonomy.
To better maintain the structure of the existing taxonomy, Shen \emph{et al.}\cite{shen2020taxoexpan} propose position-enhanced graph neural networks to encode the relative position of terms and improve the overall quality of taxonomy.
Song \emph{et al.}\cite{song2021should} design a concept sorting model to extract hyponymy relations and sort their insertion order by utilizing the relationship between the newly mined concepts.
Wang \emph{et al.}\cite{wang2021enquire} utilize the hierarchical information of the existing taxonomy by extracting tree-exclusive features in the taxonomy for better taxonomy coherence. 
One limitation of these approaches is that they mainly focus on the general-purpose taxonomies or utilize the general text corpora. Thus, they cannot be easily generalized to specific taxonomies.
Mao \emph{et al.}\cite{mao2020octet} leverage heterogeneous sources of signals such as lexical semantics and structural information to train an end-to-end online catalog taxonomy enrichment model.
The structural information is captured by modeling the structure of the core taxonomy and the query-item-taxonomy interaction in user behavior. However, it has to work with extra item-category information and cannot represent the semantics of new concepts.
Compared with these methods, our proposed method designs relational and structural representations learned from user-generated content and user click logs to model the semantics of in-domain concepts.

Study like \cite{cheng2022learning} have done the candidate query filtering, but their filtering method is mainly based on user generated content.
In our work, we formulate the task of taxonomy entering, and use generative model to self-supervised generate graph-level negative samples, which boost both the performance of traditional taxonomy expansion and the taxonomy entering.

\subsection{Text GAN}
The GANs in discrete domains encounter a problem in propagating the gradient into the generator.
SeqGAN\cite{yu2017seqgan} has overcome this problem by using a REINFORCE-like\cite{williams1992simple} algorithm in the training of the generator.
It assumes the generator as an agent that receives more reward from the discriminator to generate more realistic sentences and uses the Monte Carlo tree search to estimate the expected reward.
RankGAN\cite{juefei2018rankgan} proposes a ranking model to replace the original binary classifier as the discriminator.
LeakGAN\cite{guo2018leakgan} designs a mechanism to provide intermediate information about text generation for generator, where the discriminator can leak its features through a manager module.
MaskGAN\cite{lee2020maskgan} introduces an actor-critic conditional GAN that fills in missing text conditioned on the surrounding context by resorting to a seq2seq model.
FM-GAN\cite{amodio2021fmgan} proposes to match the latent feature distributions of real and synthetic sentences using the feature-movers distance.
REL-GAN\cite{nie2018relgan} incorporates a relational memory as a new component for modeling the long-distance dependency.
Furthermore, its discriminator utilizes multiple representations to preapre a more informative signal for the generator.

Furthermore, apart from the RL-based algorithms, very recent works, such as AutoGAN-distiller\cite{fu2020autogan}, AdversarialNAS\cite{gao2020adversarialnas}, DEGAS\cite{doveh2021degas} and alphaGAN\cite{tian2020alphagan}, employ the gradient-based algorithm to search the GAN architecture. 
It is noteworthy that gradient-based frameworks could better search generator and discriminator by playing a two-player min-max game at the same time to achieve good results. 
Kobayashi \emph{et al.}\cite{shi2022multi} adopted the evolutionary algorithm to search GAN and also achieved better results than the manual design. 
Zhou \emph{et al.}\cite{zhou2020searching} successfully applied gradient-based GANAS algorithm to the conditional GAN search.


